RF-CHORD: Towards Deployable RFID Localization System for Logistics Network

RFID localization is considered the key enabler of automating the process of inventory tracking and management for high-performance logistic network. A practical and deployable RFID localization system needs to meet reliability, throughput, and range requirements. This paper presents RF-Chord, the first RFID localization system that simultaneously meets all three requirements. RF-Chord features a one-shot multisine-constructed wideband design that can process RF signal with a 200 MHz bandwidth in real-time to facilitate one-shot localization at scale. In addition, multiple SINR enhancement techniques are designed for range extension. On top of that, a kernel-layer-based near-field localization framework and a multipath-suppression algorithm are proposed to reduce the 99% long-tail errors. Our empirical results show that RF-Chord can localize more than 180 tags 6 m away from a reader within 1 second and with 99% long-tail error of 0.786 m, achieving a 0% miss reading rate and ~0.01% cross-reading rate in the warehouse and fresh food delivery store deployment.

==> Makefile <==
TEXFILES = $(wildcard *.tex)
BIBFILES = $(wildcard *.bib)
pdflatex = pdflatex --interaction=nonstopmode --file-line-error
# initial target files
TARGETS=RF-Chord

all: $(TARGETS).pdf # a.pdf b.pdf

# initial aux file generation
# Maintain the multiple file dependencies here.
RF-Chord.aux: RF-Chord.tex\
00-abstract.tex\
01-intro.tex\
02-system_overview.tex\
03-related.tex\
03-sys-oneshot.tex\
04-sys-longrange.tex\
06-sys-alg.tex\
07-impl.tex\
08-eval.tex\
09-concl.tex\
09.1-discuss.tex\
10-proofs.tex\
11-ack.tex\
preamble.tex
	$(pdflatex) $< -draftmode
	-rm $(TARGETS).pdf

# bbl file generation
%.bbl: %.aux
	bibtex --min-crossrefs=20 $*

# pdf output  %%.bbl $(TEXFILES) $(BIBFILES) *.cls 
%.pdf: %.tex %.bbl
	$(pdflatex) $< -draftmode
	$(pdflatex) $<
	-rm  *.aux *.log  *.blg *.out *.synctex.gz *.dvi *.ps *~ *.lot *.lof *.toc
	-cp $@ /mnt/e/Documents/alii/UHFpaper/bin/


clean:
	-rm $(TARGETS).pdf *.aux *.log  *.blg *.out *.synctex.gz *.dvi *.ps *~ *.lot *.lof *.toc

